Finite Sample Analysis of Minimax Offline Reinforcement Learning: Completeness, Fast Rates and First-Order Efficiency

We offer a theoretical characterization of off-policy evaluation (OPE) in reinforcement learning using function approximation for marginal importance weights and $q$-functions when these are estimated using recent minimax methods. Under various combinations of realizability and completeness assumptions, we show that the minimax approach enables us to achieve a fast rate of convergence for weights and quality functions, characterized by the critical inequality \citep{bartlett2005}. Based on this result, we analyze convergence rates for OPE. In particular, we introduce novel alternative completeness conditions under which OPE is feasible and we present the first finite-sample result with first-order efficiency in non-tabular environments, i.e., having the minimal coefficient in the leading term.

==> def_annals.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
%\usepackage{subcaption}
%\usepackage{caption}
\usepackage{mathtools}
\usepackage{booktabs}
\usepackage{bm}
\usepackage{tcolorbox}
\usepackage{multicol,multirow}
\PassOptionsToPackage{authoryear,sort}{natbib}
\usepackage{comment}
\newcommand{\cu}{\mathcal{U}}
\newcommand{\blockedit}{\color{black}}
%\newcommand{\blockedit}{\color{magenta}}
\newcommand{\Tcal}{\mathcal{T}}
\usepackage{booktabs}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\eg}{\textit{e.g.}}
\usepackage{array}
\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\usepackage{arydshln}

\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Ie}{\textit{I.e.}}
\newcommand{\Eg}{\textit{E.g.}}
\usepackage{enumerate}   
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{bbm}
\usepackage{tikz}
\def\checkmark{\tikz\fill[scale=0.4](0,.35) -- (.25,0) -- (1,.7) -- (.25,.15) -- cycle;}
\definecolor{mygreen}{rgb}{0,0.6,0}
%\usetikzlibrary{arrows,positioning,decorations.markings}
\usetikzlibrary{positioning,arrows,decorations,decorations.markings,shadows,positioning,arrows.meta,matrix,fit}

\usetikzlibrary{positioning,arrows}
\usepackage{wrapfig}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\usepackage{amsmath}
\usepackage{appendix}
\usepackage{amssymb}

\newcommand{\lbl}[1]{\label{#1}{\ensuremath{^{\fbox{\tiny\upshape#1}}}}}
\renewcommand{\lbl}[1]{\label{#1}}

\usepackage{amsthm}
\usepackage{hyperref}
\usepackage[capitalise]{cleveref}
\Crefname{assumption}{Assumption}{Assumptions}
\crefname{lemma}{lemma}{lemmas}
\Crefname{lemma}{Lemma}{Lemmas}



\makeatletter
\def\cref@getref#1#2{%
  \xdef\@lastusedlabel{#1}%
  \expandafter\let\expandafter#2\csname r@#1@cref\endcsname%
  \expandafter\expandafter\expandafter\def%
    \expandafter\expandafter\expandafter#2%
    \expandafter\expandafter\expandafter{%
      \expandafter\@firstoftwo#2}}%

\newcommand\enameref[1]{%
  \expandafter\ifx\csname r@#1\endcsname\relax
  ??\typeout{^^JLaTeX Warning: Reference #1 undefined on input line \the\inputlineno}%
  \else
    \expandafter\expandafter\expandafter\@thirdoffive\csname r@#1\endcsname
  \fi
}    

\Crefformat{lemma}{%
    \IfStrEq{\enameref{\@lastusedlabel}}{}{%
        \Cref@lemma@name~#1%
    }{%
        \nameref{\@lastusedlabel} (#1)%
    }%
}

\crefformat{lemma}{%
    \IfStrEq{\enameref{\@lastusedlabel}}{}{%
        \cref@lemma@name~#1%
    }{%
        \nameref{\@lastusedlabel} (#1)%
    }%
}
\makeatother













%\newtheorem{theorem}{Theorem}
%\newtheorem{lemma}{Lemma}
%\newtheorem{example}{Example}

%
%
\DeclareMathOperator*{\plim}{plim}
\usepackage{graphicx}
\newcommand{\indep}{\rotatebox[origin=c]{90}{$\models$}}
\newcommand{\iid}{ \stackrel{i.i.}{\sim} }
\newcommand{\bx}{\mathbf{x}}
\newcommand{\btau}{\mathbf{\tau}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bpi}{\pmb{\pi}}
\newcommand{\bh}{\mathbf{\pi}}
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\con}{concentratability\,}
\newcommand{\rea}{realizability\,}
\newcommand{\real}{realizability\,}
\newcommand{\comp}{completeness\,}
\newcommand{\smallo}{{\scriptscriptstyle\mathcal{O}}} %
\newcommand{\bo}{\mathbf{0}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bG}{\mathbb{G}}
\def\Holder{{H\"{o}lder}}
\newcommand{\bu}{\mathbf{u}}
\def\Cramer{Cram\'{e}r}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\nhs}{n^{\mathrm{hst}}}
\newcommand{\fix}{\mathrm{fix}}
\newcommand{\nev}{n^{\mathrm{evl}}}
\newcommand{\EB}{\mathrm{EB}}
\newcommand{\para}{\mathrm{para}}
\newcommand{\CK}{\mathrm{ck}}
\newcommand{\OP}{\mathrm{op}}
\newcommand{\CD}{\mathrm{cd}}
\newcommand{\MK}{\mathrm{mk}}
\newcommand{\MD}{\mathrm{md}}
\newcommand{\MDL}{\mathrm{mdl}}
\newcommand{\MIL}{\mathrm{mil}}
\newcommand{\MFL}{\mathrm{mfl}}
\newcommand{\MABO}{\mathrm{mabo}}
\newcommand{\bN}{\mathcal{N}}
\newcommand{\noo}{N_o}
\newcommand{\oO}{\mathcal{O}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\cm}{\mathcal{M}}
\newcommand{\MDP}{\mathrm{MDP}}
\newcommand{\MSE}{\mathrm{MSE}}
\newcommand{\ch}{\mathcal{H}}
\newcommand{\bigO}{\mathcal{O}} %
\newcommand{\cj}{\mathcal{J}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\oper}{\mathrm{op}}
\newcommand{\ts}{\textstyle}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\CR}{\mathrm{CR}}
\newcommand{\te}{\mathrm{te}}
\newcommand{\VC}{\mathrm{VC}}
\newcommand{\case}{\mathrm{case}}
\newcommand{\buu}{\mathbf{u}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\hP}{\mathbb{P}_n}
\newcommand{\hG}{\mathbb{G}}
\newcommand{\Op}{\mathrm{O}_{p}}
\newcommand{\op}{\mathrm{o}_{p}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Pa}{\mathrm{Pa}}
\newcommand{\pa}{\mathrm{\pa}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\calh}{\mathcal{H}}
\newcommand{\rI}{\mathrm{I}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\var}{\mathrm{var}}
\newcommand{\cov}{\mathrm{cov}}
\newcommand{\rE}{\mathrm{E}}
\newcommand{\thpol}{\pi^{\theta}}
\newcommand{\thhatpol}{\pi^{\hat{\theta}}}
\newcommand{\rvar}{\mathrm{var}}
\newcommand{\Asmse}{\mathrm{Asmse}}
\newcommand{\dml}{\mathrm{DRCS}}
\newcommand{\dm}{\mathrm{DM}}
\newcommand{\rD}{\mathrm{d}}
\newcommand{\rd}{\mathrm{d}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\htheta}{\hat{\theta}}
\newcommand{\prns}[1]{\left(#1\right)}
\newcommand{\braces}[1]{\left\{#1\right\}}
\newcommand{\bracks}[1]{\left[#1\right]}
\newcommand{\braangle}[1]{\langle#1\rangle}
\newcommand{\branormal}[1]{(#1)}
\newcommand{\sumT}{\sum_{t=0}^T}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\Rl}{\mathbb{R}}
\newcommand{\R}[1]{\mathbb{R}^{#1}}
\newcommand{\epol}{\pi^\mathrm{e}}
\newcommand{\bpol}{\pi^{\mathrm{b}}}
\newcommand{\bpolh}{\hat \pi^b}
\newcommand{\FI}{\mathrm{FI}}
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\pre}{\mathrm{pre}}
\newcommand{\tmle}{\mathrm{tmle}}
\newcommand{\ipw}{\mathrm{IPW}}
\newcommand{\DM}{\mathrm{DM}}
\newcommand{\dr}{\mathrm{DR}}
\newcommand{\prepi}[1]{d_0 \times #1}
\newcommand{\ini}{p_{\mathrm{ini}}}
\newcommand{\opera}{p_{\mathrm{op}}}
\newcommand{\inipi}[1]{p_{\mathrm{ini}, #1}}
\newcommand{\magd}[1]{\left\|#1\right\|}
\newcommand\ci{\perp\!\!\!\perp}
\newcommand{\Rfrak}{\mathfrak{R}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Abbb}{\mathbb{A}}
\newcommand{\Bbbb}{\mathbb{B}}
\newcommand{\Rbbb}{\mathbb{R}}
\newcommand{\Wbbb}{\mathbb{W}}
\newcommand{\Qbbb}{\mathbb{Q}}
\newcommand{\Vbbb}{\mathbb{V}}
\newcommand{\Ubbb}{\mathbb{U}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Zcal}{\mathcal{Z}}
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\MWL}{\mathrm{mwl}}
\newcommand{\MQL}{\mathrm{mql}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Error}{\mathrm{Err}}
% Macros for the MWQL paper

\newcommand{\Lw}{L_{\mathrm{w}}}
\newcommand{\Lwn}{L_{\mathrm{w},n}}
\newcommand{\Lq}{L_{\mathrm{q}}}
\newcommand{\Lqn}{L_{\mathrm{q},n}}
\newcommand{\hatw}{\hat{w}}
\newcommand{\hatwn}{\hat{w}_n}
\newcommand{\hatq}{\hat{q}}
\newcommand{\hatqn}{\hat{q}_n}
\newcommand{\Rw}{R_{\mathrm{w}}}
\newcommand{\Rwn}{R_{\mathrm{w},n}}
\newcommand{\Rq}{R_{\mathrm{q}}}
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}

\renewcommand{\eqref}[1]{(\ref{#1})}

\newcommand{\bepsilon}{{\mbox{\boldmath$\epsilon$}}}
\newcommand{\RN}[1]{%
  \textup{\uppercase\expandafter{\romannumeral#1}}%
}
\newcommand{\bmu}{{\mbox{\boldmath$\mu$}}}

\newcommand{\bbeta}{{\mbox{\boldmath$\beta$}}}

\usepackage{color,graphicx,lscape,longtable}

\def\boxit#1{\vbox{\hrule\hbox{\vrule\kern6pt\vbox{\kern6pt#1\kern6pt}\kern6pt\vrule}\hrule}}
\def\macomment#1{\vskip 2mm\boxit{\vskip 2mm{\color{red}\bf#1}
    {\color{blue}\bf -- MA\vskip 2mm}}\vskip 2mm}

\def\jkcomment#1{\vskip 2mm\boxit{\vskip 2mm{\color{red}\bf#1}
    {\color{blue}\bf -- J.K. \vskip 2mm}}\vskip 2mm}

\usepackage{xcolor}
\newcount\Comments  % 0 suppresses notes to selves in text
\Comments=1 % TODO: change to 0 for final version
\newcommand{\kibitz}[2]{\ifnum\Comments=1\textcolor{#1}{#2}\fi}
\newcommand{\masa}[1]{\kibitz{red}{[MU: #1]}}
\newcommand{\txie}[1]{\kibitz{cyan}{[TX: #1]}}
\newcommand{\nk}[1]{\kibitz{magenta}{[NK: #1]}}
\newcommand{\imaizumi}[1]{\kibitz{blue}{[MI: #1]}}
% comment Tengyang
\newcommand{\Pcal}{\mathcal{P}}


==> main_file/main_intro.tex <==
%!TEX root = ../colt2021_main.tex

 Off-policy evaluation (OPE) is the problem of estimating the expected return in an unknown Markov decision process (MDP) of a given decision policy, known as the evaluation policy, using transition data generated by another policy, known as the behavior policy \citep{Precup2000,pmlr-v37-thomas15,pmlr-v97-bibaut19a,LevineSergey2020ORLT,NamkoongHongseok2020OPEF,ShiChengchun2021DOIE,MaCong2021MOEf}. OPE is especially important in applications where experimentation is particularly costly, such as in medicine \citep{LuckettDanielJ.2018EDTR,2019PM,chakraborty2013statistical} and in education \citep{Mandel2014}. Recently, the first-order efficiency bound for OPE was derived by \citep{KallusUehara2019} for time-varying MDPs and by \citep{KallusNathan2019EBtC} for time-homogeneous MDPs (which we focus on and simply call MDPs). That is, the smallest-possible coefficient of the leading $1/\sqrt{n}$ term $C$ in the estimation error $\ts C/\sqrt{n} + o(1/\sqrt{n}).$ In the time-varying tabular setting, the bounds coincides with that of \citep{jiang}, and \citep{YinMing2020AEOE} showed that the model-based estimator achieves it. However, the achievability of the lower bound in general settings is unclear.

Among the approaches to OPE, many of them rely on estimating the $q$-function (representing the long-term value of a given state-action pair) or the $w$-function (representing density ratios of the state occupancy measures), under the so-called \emph{realizability} (a.k.a~well-specification) and/or \emph{completeness} (a.k.a~hypothesis class closed under Bellman operators; \citep{antos2008learning}) assumptions. For example, the $q$-function can be estimated via Fitted-Q Iteration (FQI) and it is known it has a valid finite-sample guarantee under the completeness and realizability \citep{ChenJinglin2019ICiB,munos2008finite}. The $w$-function is central to recent methods based on the idea of marginalized importance sampling \citep{Liu2018,edsarx.1901.0945520190101}; however, it is less understood when it has a convergence guarantee. 

In this paper, we study minimax estimators of $q$- and $w$-functions and its implications for OPE. These estimators take the form of solutions to zero-sum games between $q$ and $w$. Related estimators have been proposed for $w$- \citep{NachumOfir2019APGf,zhang2019gendice,UeharaMasatoshi2019MWaQ} and $q$-functions \citep{antos2008learning,FengYihao2019AKLf,UeharaMasatoshi2019MWaQ}, but their statistical properties are not well understood or tightly characterized. 
Here, we develop \emph{fast} rates of convergence for these estimators under a variety of realizability and completeness conditions, many of which are new.
Furthermore, we show how this leads to OPE with finite-sample guarantees that enjoy first-order efficiency, meaning having the minimal leading term.

We next give a brief overview of our results, also summarized in \cref{tab:summary}:
\begin{itemize}
   \item (\RNum{1} in  \cref{tab:summary}: \cref{sec:without_sta}) Under $q$- and $w$-realizability, we derive rates of convergence of the minimax approach by refining the analysis of \cite{UeharaMasatoshi2019MWaQ}. 
   \item (\RNum{2},\RNum{3},\RNum{4},\RNum{5} in  \cref{tab:summary}: \cref{sec:fast_slow,sec:without_sta_rate}) Under a variety of completeness assumptions, we show the minimax approach enables us to achieve a fast rate of convergence for $q$- and $w$-functions, characterized by the critical inequality based on localized Rademacher complexity \citep{bartlett2005}. This is the \emph{first} finite-sample result obtaining a fast rate for $w$-functions and it introduces novel completeness assumptions. This is also the \emph{first} finite-sample result obtaining a fast rate for $q$-functions when using minimax estimators with general function approximation. 
   We apply these results to derive the rate for OPE, which is generally slower than the case in \RNum{1}. 
    \item (\RNum{6} in \cref{tab:summary}: \cref{sec:efficiency}) Under both \rea and completeness of both $w$- and $q$-functions, we present the \emph{first} finite sample result that indicates the first-order lower bound is achieved in non-tabular environments. Our result covers a tabular case as a special case.\footnote{Strictly speaking, our tabular result is also a new result since \citep{YinMing2020AEOE} discusses a model based estimator on time-varying MDPs. Our setting is time-homogeneous MDP.} 
    \item  (\cref{sec:extension}) In \cref{tab:summary}, we have focused on the state-action based minimax estimators. Here, we extend our analysis in \cref{tab:summary} to the following two cases: (1) state-based minimax estimators \citep{Liu2018,FengYihao2019AKLf}, (2) policy optimization \citep{XieTengyang2020QASf}. 
\end{itemize}
Note all of the proofs are in \cref{ape:proof}. Comparison to other work is discussed in \cref{sec:comparison}.  

\begin{table}[t!]
    \centering
\caption{The rates of our finite-sample bounds on $|\hat J^{\MIL}-J|$ under different assumptions where $\hat J^{\MIL}$ is an estimator for OPE based on nuisance estimators $\hat w_{\epol},\hat q_{\epol}$. The hypothesis classes $\Wbbb_1,\Qbbb_1$ are used to estimate $w_{\epol}$ and $\Wbbb_2,\Qbbb_2$ to estimate $q_{\epol}$. We summarize our conclusions for the cases of VC classes or
Sobolev balls $H^{\alpha,d}$ of $\alpha$-times differentiable functions of $d$-dimensional inputs.
Dependence on $1/(1-\gamma),C_{w},R_{\max},C_{\xi},\log(1/\delta)$ are polynomial, where $C_w$ is a distribution mismatch coefficient. ``Sta" refers to whether we use stabilizers. Note the rate in \RNum{6} is faster than the one in \RNum{1}, which is faster than the ones in \RNum{2}, \RNum{3}, \RNum{4}, \RNum{5}.  
 }
    \begin{tabular}{m{0.018\textwidth}m{0.232\textwidth}m{0.05\textwidth}m{0.30\textwidth}m{0.30\textwidth}}\toprule
         & Main Assumptions  &  Sta & Rates  (ignoring $\log n$) &  Note   \\ \midrule
       \RNum{1} & {\small $w_{\epol}\in \Wbbb_1,\,q_{\epol}\in \Qbbb_1$  or  $w_{\epol}\in \Wbbb_2,\,q_{\epol}\in \Qbbb_2$}  &  No &  $n^{-1/2}~~(\mathrm{VC})$\hfill\break$\max(n^{-1/2},\,n^{-\alpha/d})~~(H^{\alpha,d} )$   & \\  \hline
       \multirow{ 2}{*}{\RNum{2}} &    {\small $q_{\epol}\in \Qbbb_2$  \hfill\break$C_{\xi}T_{\gamma}(\Qbbb_2-q_{\epol})\subset\Wbbb_2$} &  No  &  $n^{-1/4}~~(\mathrm{VC})$\hfill\break$\max(n^{-1/4},\,n^{\frac{-\alpha}{2d}})~~(H^{\alpha,d})$\hfill\break    &     We obtain a guarantee for $\|\Bcal\hat q-\hat q\|_2$. 
     The condition and rate (with sta) are the same as FQI.     \\   
      &   & Yes  & $n^{-1/2} (\mathrm{VC})$\hfill\break$\max(n^{-1/2},\,n^{-\frac{\alpha}{2\alpha+d}})~~(H^{\alpha,d})$    &  \\ \hline
       \RNum{3}  &     {\small $q_{\epol}\in \Qbbb_2$,\hfill\break$C_{\xi}(\Qbbb_2-q_{\epol})\subset T'_{\gamma}\Wbbb_2 $} &  Yes/No   &  Same as the above     &  We obtain a guarantee for $\|\hat q-q_{\epol}\|_2$.     \\  \hline
           \RNum{4}  & {\small $w_{\epol}\in \Wbbb_1$,\hfill\break$C_{\xi}(\Wbbb_1-w_{\epol})\subset T_{\gamma}\Qbbb_1 $}  &  Yes/No   &  Same as the above    &  We obtain a guarantee for $\|\hat w-w_{\epol}\|_2$    \\  \hline
       \RNum{5} &     {\small $w_{\epol}\in \Wbbb_1$,\hfill\break$C_{\xi}T'_{\gamma}(\Wbbb_1-w_{\epol})\subset \Qbbb_1$} & Yes/No    &  Same as the above    &  We obtain a guarantee for $\|\Bcal'\hat w-\hat w\|_2$    \\  \hline
       \RNum{6} &  {\footnotesize $q_{\epol}\in \Qbbb_2,\,w_{\epol}\in \Wbbb_1$,\hfill\break$C_{\xi}T_{\gamma}(\Qbbb_2-q_{\epol})\subset \Wbbb_2$,\hfill\break$C_{\xi} T'_{\gamma}(\Wbbb_1-w_{\epol})\subset\Qbbb_1$} &  Yes  & $n^{-1/2}~~(\mathrm{VC})$\hfill\break$\max(n^{-1/2},\,n^{\frac{-2\alpha}{2\alpha+d}})~~(H^{\alpha,d})$   &
     Our OPE error bound is first-order efficient in the cases where the rate is $n^{-1/2}$. \\\bottomrule
    \end{tabular}
\label{tab:summary}

\end{table}


==> proof/proof_error.tex <==
%!TEX root = ../colt2021_main.tex

In this section, We often use the following lemmas. 
\begin{lemma}[Dudley integral]\label{lem:dudley}
\begin{align*}
    \Rcal_n(\Fcal)\lesssim \inf_{\tau\geq 0}\braces{\tau+\int_{\tau}^{\sup_{f\in \Fcal}\sqrt{\E_n[f^2]}}\sqrt{\frac{\log \Ncal(\tau,\Fcal,\|\cdot\|_n)}{n}}}. 
\end{align*}
\end{lemma}
Note $\sup_{f\in \Fcal}\sqrt{\hP[f^2]}$ is upper bounded by the envelope $\|\Fcal\|_{\infty}$.
\begin{lemma}{\citet[Corollary 14.3]{WainwrightMartinJ2019HS:A}}\label{lem:critical_basic}
        Let $\Ncal(\tau;\mathbb{B}(\delta;\Fcal),\|\cdot\|_n)$ denote the $\tau$-covering number of $\mathbb{B}_n(\delta;\Fcal):=\{f| \|f\|_n\leq \delta\}$. Then, the critical inequality of the empirical version is satisfied for any $\delta>0$ s.t.
        \begin{align*}
            \frac{1}{\sqrt{n}}\int^{\delta}_{\delta^2/(2\|\Fcal\|_{\infty})}\sqrt{\log  \Ncal(t,\mathbb{B}_n(\delta;\Fcal),\|\cdot\|_n)}\rd t\leq \frac{\delta^2}{\|\Fcal\|_{\infty}}.
        \end{align*}
\end{lemma}


\begin{proof}[Proof of Lemma \ref{lem:covering_G}]
Fix $\varepsilon_1 > 0$ and $\varepsilon_2>0$ and set $N_Q = \bN(\varepsilon_1, \Qbbb, \|\cdot\|_\infty)$ and $N_W = \bN(\varepsilon_2, \Wbbb, \|\cdot\|_\infty)$.
We pick an $\varepsilon_1$-covering set $\{q_i\}_{i=1}^{N_Q} \subset \Qbbb$, that is, for any $q \in \Qbbb$, there exists $q_i \in \{q_i\}_{i=1}^{N_Q} $ such as $\|q - q_i\|_\infty \leq \varepsilon_1$.
Similarly, we pick an $\varepsilon_2$-covering set $\{w_j\}_{j=1}^{N_W} \subset \Wbbb$.

We consider a functional $G: \Wbbb \times \Qbbb \to \Gcal$ such as
\begin{align*}
	G[w,q](s,a,r,s') := w(s,a)\{-q(s,a)+\gamma  \rE_{a' \sim \pi_e(a'|s')}[q(s',a')]\}.
\end{align*}
Simply, we have $\Gcal = \{G[w,q] ; w\in \Wbbb,q\in \Qbbb \}$.
Using the picked covering set, we consider a finite set $\tilde{\Gcal} := \{G[w_j,q_i] ; i = 1,...,N_Q, j = 1,...,N_W \} \subset \Gcal$.
Obviously, we have $|\tilde{\Gcal} |\leq N_W N_Q$.


We will show that $\tilde{\Gcal}$ is a covering set of $\Gcal$.
Pick $G[w,q] \in \Gcal$ arbitrary, then we can pick $w_j$ and $q_i$ such as $\|q-q_i\|_\infty \leq \varepsilon_1$ and $\|w-w_j\|_\infty \leq \varepsilon_2$.
Then, we evaluate $G[w_j,q_i] (s,a,r,s')- G[w,q](s,a,r,s')$ as
\begin{align*}
	&|G[w_j,q_i] (s,a,r,s')- G[w,q](s,a,r,s') |\\
	& = |w_j(s,a)\{-q_i(s,a)+\gamma  \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a')]\} - w(s,a)\{q(s,a)+\gamma  \rE_{a' \sim \pi_e(a'|s')}[q(s',a')]\} | \\
	&=|(w_j(s,a) - w(s,a))\{-q_i(s,a)+\gamma  \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a')]\} \\
	&  \quad + w(s,a)[-(q(s,a) - q_i(s,a)) + \gamma ( \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a')] -  \rE_{a' \sim \pi_e(a'|s')}[q(s',a')])]| \\
	& \leq |w_j(s,a) - w(s,a)| |-q_i(s,a)+\gamma  \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a')]| \\
	& \quad + |w(s,a)| |-(q(s,a) - q_i(s,a)) + \gamma ( \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a') - q(s',a')])| \\
	& =: I + II.
\end{align*}
We bound the terms $I$ and $II$ separately.
For the first term $I$, we have
\begin{align*}
	I&\leq |w_j(s,a) - w(s,a)| (|q_i(s,a)| + |\gamma  \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a')]||) \\
	& \leq \|w_j - w\|_\infty ( \|q_i\|_\infty + \gamma \|q_i\|_\infty) \leq \varepsilon_2  (1+\gamma) C_\Qbbb.
\end{align*}
For the second term $II$, we have
\begin{align*}
	II &\leq \|w\|_\infty (|q(s,a) - q_i(s,a)| + \gamma | \rE_{a' \sim \pi_e(a'|s')}[q_i(s',a') - q(s',a')]| ) \\
	&\leq C_\Wbbb (\|q-q_i\|_\infty + \gamma \|q-q_i\|_\infty) \leq C_\Wbbb (1+\gamma) \varepsilon_1.
\end{align*}

Combining the bound, we find that $\tilde{\Gcal}$ is a $(\varepsilon_2  (1+\gamma) C_\Qbbb + C_\Wbbb (1+\gamma) \varepsilon_1)$-covering set of $\Gcal$.
That is, we have
\begin{align*}
	\bN(\varepsilon_2 ( (1+\gamma) C_\Qbbb) + C_\Wbbb (1+\gamma) \varepsilon_1, \Gcal, \|\cdot\|_\infty) \leq N_Q N_W = \bN(\varepsilon_1, \Qbbb, \|\cdot\|_\infty)\bN(\varepsilon_2, \Wbbb, \|\cdot\|_\infty).
\end{align*}
Substituting $\varepsilon_2 = 0.5\varepsilon/ ((1+\gamma) C_\Qbbb)$ and $\varepsilon_1 = 0.5\varepsilon/(C_\Wbbb (1+\gamma))$ yields the statement.
\end{proof}


%\begin{proof}[Proof of Lemma \ref{lem:covering_linear}]
%For any parameter vectors $\theta_w,\theta'_w\in \mathbb{R}^{d_1}$, we have
%\begin{align*}
%    |\theta_w^\top \phi(s,a) - (\theta'_w)^\top \phi(s,a)| = |(\theta_w - \theta'_w)^\top \phi(s,a)| \leq \|\theta'_w - \theta_w\|_1,
%\end{align*}
%by the \Holder's inequality. By this result, we obtain that
%\begin{align*}
%    \Ncal(\varepsilon, \Wbbb, \|\cdot\|_\infty) \leq \Ncal( \varepsilon, \{w_K : \|w_K\|_1\leq \kappa_1\}, \|\cdot\|_1) \leq \left(1 +  \frac{\kappa_1}{ \varepsilon}\right)^{d_1}.
%\end{align*}
%For $\Qbbb$, the same discussion yields the statement.
%\end{proof}
%
%\begin{proof}[Proof of Corollary \ref{cor:linear_order}]
%By combining Lemma \ref{lem:covering_G} and Lemma \ref{lem:covering_linear}.
%%\begin{align*}
%        \bN(\varepsilon, \Gcal(\Wbbb,\Qbbb), \|\cdot\|_\infty) \leq \left(1 +  \frac{\kappa_1 (1+\gamma) \kappa_2 )}{ \varepsilon}\right)^{d_1}\left(1 +  \frac{\kappa_1 \kappa_2 (1+\gamma)}{ \varepsilon}\right)^{d_2}.
%  \end{align*}
%Note that $C_\Qbbb = \kappa_2 $ and $C_\Wbbb = \kappa_1.$ The final statement holds by calculating Dudley integral. 
%
%\end{proof}


\begin{proof}[Proof of Corollary \ref{cor:vc_classes}]
~
\paragraph{First part}
First, we prove that the VC dimension of $\Vbbb\coloneqq \{q(s,\epol);q\in \Qbbb\}$ is upper-bounded by $V(\Qbbb)$. Consider the set of subgraphs of $\Vbbb$ as $\mathcal{V}$. Then, we take $n$ points $s_1,\cdots,s_n$ shattered by $\Vbbb$. This states for any binary sequence $\{b_1,\cdots,b_n\}$, there exists $v' \in \Vbbb$ and $t' \in \mathbb{R}$ s.t. 
\begin{align*}
    \rI(q_{v'}(s_1,\epol) - t' >0)=b_1,\cdots,     \rI(q_{v'}(s_n,\epol) - t'>0)=b_n,
\end{align*}
where $q_{v'} \in \Qbbb$ is a corresponding function such as $v'(s)=q_{v'}(s,\epol)$.
%\imaizumi{I introduced $t' \in \mathbb{R}$ to follow the definition of subgraph. Is it OK?}
We, then, consider the set of subgraphs of $\Qbbb$ as $\mathcal{Q}$, and show that $\mathcal{Q}$ can shatter $(s_1,a_1),...,(s_n,a_n)$ associated with $s_1,...,s_n$.
To bound the VC dimension of $\Vbbb$, it is sufficient to show
\begin{align}
    \exists a, ~\mathrm{sign}(q_{v'}(s,\epol) - t') = \mathrm{sign}(q_{v'}(s,a) - t'), \label{eq:sign_q}
\end{align}
holds for any $s$.
To show \eqref{eq:sign_q}, without loss of generality, we assume $q_{v'}(s,\epol) \geq t'$, which is equivalent to
\begin{align}\label{eq:contra}
    \ts \int q_{v'}(s,a)\epol(a|s)\rd(a)>t'. 
\end{align}
We use the contradiction argument. Suppose there is no $a\in \Acal$ s.t. $ q_{v'}(s,a)>t'$, then 
\begin{align*}
   \ts  \int q_{v'}(s,a)\epol(a|s)\rd(a)\leq t',
\end{align*}
holds. 
This contradicts \cref{eq:contra}, hence there exists $a\in \Acal$ s.t. $      q_{v'}(s,a)>t' $.
%\imaizumi{I do not fully sure whether \eqref{eq:sign_q} holds. If we can set $t '= 0$, the same question may appear.}
Hence, we can take $\{a_1,\cdots,a_n\}$ as satisfying \eqref{eq:sign_q} for each $s_1,...,s_n$ and obtain
\begin{align*}
    \rI(q_{v'}(s_1,a_1) - t'>0)=b_1,\cdots,  \rI(q_{v'}(s_n,a_n) - t'>0)=b_n. 
\end{align*}
This concludes that $V(\Vbbb)\leq V(\Qbbb)$.

\paragraph{Second part}
\begin{align*}
    \Rcal_n(\Gcal(\Wbbb,\Qbbb))&= \Rcal_n(\Wbbb \Qbbb )+\gamma \Rcal_n(\Wbbb \Vbbb )\\ 
    &\leq 0.25\{\Rcal_n((\Wbbb+\Qbbb)^2-(\Wbbb-\Qbbb)^2 )+\gamma \Rcal_n((\Wbbb+\Vbbb)^2-(\Wbbb-\Vbbb)^2 )\} \\ 
    &\leq \{C_{\Wbbb}C_{\Qbbb}\Rcal_n(\Wbbb+\Qbbb))+\gamma  C_{\Wbbb}C_{\Qbbb}\Rcal_n(\Wbbb+\Vbbb)\}\tag{Contraction property \citep{mendelson2002improving}} \\ 
\end{align*}
Here, we have 
\begin{align*}
    \Rcal_n(\Wbbb)&\ts =\int_{0}^{C_{\Wbbb}}\sqrt{\log \Ncal(t,\Wbbb,\|\cdot\|_n)/n}\rd(t)\\
    &\ts =O\braces{ \int_{0}^{C_{\Wbbb}}\sqrt{V(\Wbbb)\log(1/t) /n}\rd(t)   }\\
    &\ts=O(\sqrt{V(\Wbbb)/n}). 
\end{align*}
The covering number is calculated using \citet[Lemma 19.15]{VaartA.W.vander1998As}, that is, for a VC class of functions $\Fcal$ with measurable envelope function $F$ and $r\geq 1$, one has for any probability measure $Q$ with $\|F\|_{Q,r}>0$, 
\begin{align*}
    \Ncal(\epsilon \|F\|_{Q,r},\Fcal,L_r(Q))\lesssim V(\Fcal)(4e)^{V(\Fcal)}\prns{\frac{2}{\epsilon}}^{rV(\Fcal)}. 
\end{align*}
Thus, 
\begin{align*}
       R_{\max}\Rcal_n(\Wbbb)+\Rcal_n(\Gcal(\Wbbb,\Qbbb))= O(\sqrt{(V(\Wbbb)+V(\Qbbb))/n}). 
\end{align*}
This concludes that with probability $1-\delta$, 
\begin{align*}
    |\hat J^{\MIL}-J|= O(\sqrt{(V(\Wbbb)+V(\Qbbb))/n}).
\end{align*}
\end{proof}



\begin{proof}[Proof of Corollary \ref{cor:nonpara_order}]
We have 
\begin{align*}
		&\sqrt{\log \bN(\tau, \Gcal(\Wbbb,\Qbbb), \|\cdot\|_\infty)} \\
		&\leq \sqrt{\log(0.5\tau/((1+\gamma)C_\Qbbb), \Wbbb, \|\cdot\|_\infty) + \log \bN(0.5\tau/((1+\gamma)C_\Wbbb), \Qbbb, \|\cdot\|_\infty)}\\
		 &\leq\sqrt{\log(0.5\tau/((1+\gamma)C_\Qbbb), \Wbbb, \|\cdot\|_\infty)} + \sqrt{\log \bN(0.5\tau/((1+\gamma)C_\Wbbb), \Qbbb, \|\cdot\|_\infty)}. 
\end{align*}

First, we consider the case when $\beta<2$, from Lemma \ref{lem:dudley}, the final error is 
\begin{align*}
O\prns{n^{-1/2}\braces{1-\braces{\frac{1}{\tau}}^{0.5\beta_1-1}}+\tau}. 
\end{align*}
By taking $\tau=\Theta(1/n)$, the final error is $O(n^{-1/2})$. 

Next, we consider the case when $\beta=2$.  From Lemma \ref{lem:dudley}, the final error is 
\begin{align*}
     O\prns{n^{-1/2}\{1-\log(\tau)\}+\tau}.  
\end{align*}
By taking $\tau=\Theta(\log(n)/\sqrt{n})$, the final error is $O(n^{-1/2}\log n)$. 

Finally, consider the case  when $\beta\geq 2$.  From Lemma \ref{lem:dudley}, the final error is 
\begin{align*}
O\prns{n^{-1/2}\braces{\braces{\frac{1}{\tau}}^{0.5\beta-1}-1}+\tau}. 
\end{align*}
Here, by taking $\tau=\Theta(n^{-1/\beta})$, the final error is  $O(n^{-1/\beta})$. 


\end{proof}



\begin{proof}[Proof of Corollary \ref{cor:linear_sieve}]
WLOS, we prove the case for $\hat J^{\MIL}_q$. From \cref{thm:allow_mis1}, 
\begin{align*}
|\hat J^{\MIL}_q-J|&=O(R_{\max}\Rcal_n(\Wbbb)+\Rcal_n(\Gcal(\Wbbb,\Qbbb)))\\
&+\min_{w\in \Wbbb}\max_{q \in \Qbbb}\E[(w-w_{\epol})\Tcal_{\gamma}(q-q_{\epol})]+\min_{q \in \Qbbb}\max_{w\in \Wbbb}\E[w\Tcal_{\gamma}(q-q_{\epol})]).
\end{align*}
Then, from the assumption of sieve space $\Wbbb$, we have 
\begin{align*}
 &\min_{w\in \Wbbb}\max_{q \in \Qbbb}\E[(w-w_{\epol})\Tcal_{\gamma}(q-q_{\epol})]\\
 &\lesssim \min_{w \in \Wbbb}\|w-w_{\epol}\|_{\infty}(C_{\Qbbb}+R_{\max}(1-\gamma)^{-1}) \tag{from $\|\Tcal_{\gamma}(q-q_{\epol})\|_{1}\lesssim C_{\Qbbb}+R_{\max}(1-\gamma)^{-1})$}\\
 &= O(k^{-p/d}_n). 
\end{align*}
Similarly, from the assumption of sieve space $\Qbbb$, we have 
\begin{align*}
    \min_{q \in \Qbbb}\max_{w\in \Wbbb}\E[w\Tcal_{\gamma}(q-q_{\epol})]\leq (1+\gamma)C_{\Wbbb}\min_{q \in \Qbbb}\|q-q_{\epol}\|_{\infty}= O(k^{-p/d}_n). 
\end{align*}
In addition, we have $R_{\max}\Rcal_n(\Wbbb)+\Rcal_n(\Gcal(\Wbbb,\Qbbb))= O(\sqrt{k_n/n})$ from Corollary \ref{cor:vc_classes}. In the end, the final error becomes $$O(\ts \sqrt{k_n/n}+k^{-p/d}_n).$$  Balancing these two terms, the final error is $ O(n^{-\frac{p}{2p+d}})$. 
\end{proof}

\begin{proof}[Proof of Corollary \ref{cor:neural_net}]
WLOS, we prove the case for $\hat J^{\MIL}_q$. 
As a similar discussion as the proof of Corollary \ref{cor:linear_sieve}, $ |\hat J^{\MIL}-J|$ is upper-bounded by 
\begin{align*}
&O(R_{\max}\Rcal_n(\Wbbb))+\Rcal_n(\Gcal(\Wbbb,\Qbbb))+\min_{w\in \Wbbb}\max_{q \in \Qbbb}\E[(w-w_{\epol})\Tcal_{\gamma}(q-q_{\epol})]+\min_{q \in \Qbbb}\max_{w\in \Wbbb}\E[w\Tcal_{\gamma}(q-q_{\epol})]  \tag{  \cref{thm:allow_mis1}}\\ 
&=O(R_{\max}\Rcal_n(\Wbbb))+\Rcal_n(\Gcal(\Wbbb,\Qbbb))+\tilde{O}( \Omega^{-p/ d}) \tag{Lemma \ref{lem:yaro}} \\
&=O(\Rcal_n(\mathcal{F}_{NN}))+\tilde{O}( \Omega^{-p/ d}) \tag{ Contraction property } \\
&= O\prns{\sqrt{\Omega L/n}\int_{0}^{C} \sqrt{\log(LB(\Omega+1)/t)}\rd\mu(t)}+\tilde{O}( \Omega^{-p/ d}),  \tag{Lemma \ref{lem:covering_neural} and Dudley integral}
\end{align*}
where $\Fcal_{NN}\leq C$. Then, by taking $L=\Theta(\log n),\Omega=\Theta(n^{d/(2p+d)})$, the statement is concluded.  
\end{proof}

\begin{proof}[Proof of Corollary \ref{cor:neural_net_overparam}]
WLOS, we prove the case for $\hat J^{\MIL}_q$. We define $C_{NN} := \max \{ C_\Wbbb, C_\Qbbb\} $ which is finite by the boundedness of $A_\ell$ for $\mathcal{F}_{NN}$.
As a similar discussion as the proof of Corollary \ref{cor:linear_sieve},  $    |\hat J^{\MIL}-J|$ is upper-bounded by 
\begin{align*}
      &O(R_{\max}\Rcal_n(\Wbbb))+\Rcal_n(\Gcal(\Wbbb,\Qbbb))+\min_{w\in \Wbbb}\max_{q \in \Qbbb}\E[(w-w_{\epol})\Tcal_{\gamma}(q-q_{\epol})]+\min_{q \in \Qbbb}\max_{w\in \Wbbb}\E[w\Tcal_{\gamma}(q-q_{\epol})]  \tag{  \cref{thm:allow_mis1}}\\ 
        &=O(\Rcal_n(\mathcal{F}_{NN})+\epsilon)  \tag{ Contraction property and the assumption for the approximation error}.  
\end{align*}
%By the slight update the proof of \cref{thm:generalization}, we obtain
%\begin{align*}
%    |\Hat{J}^{\mathrm{mil}} - J| &\leq O((R_{\max}C_{NN} + C_{NN}^2)\varepsilon) + R_{\max} \mathcal{R}_n(\mathcal{F}_{NN}) \\
%    & \quad + \mathcal{R}_n(\mathcal{G}(\mathcal{F}_{NN},\mathcal{F}_{NN})) + (R_{\max}C_{NN} + C_{NN}^2) \sqrt{\log(c_n/\delta)n^{-1}} \\
%    & \lesssim \varepsilon + \mathcal{R}_n(\mathcal{F}_{NN}) + \sqrt{\log(c_n/\delta)n^{-1}}.
%\end{align*}
We apply Lemma \ref{lem:golowich} and obtain the statement.
\end{proof}

%\begin{proof}[Proof of Lemma \ref{lem:linear_critical}]
%We calculate 
%\begin{align*}
%      \frac{1}{\sqrt{n}}\int^{\delta}_{0}\sqrt{\log  \Ncal(t;\mathbb{B}_n(\delta;\Wbbb(\Qbbb-q_0)),\|\cdot\|_n)}\rd t.
%\end{align*}
%This is upper bounded by 
%\begin{align*}
%    \frac{1}{\sqrt{n}}\int_0^{\delta}d_1\sqrt{\log\prns{1+\frac{\kappa_1\kappa_2(1+\gamma)}{\epsilon}}}+d_2\sqrt{\log\prns{1+\frac{\kappa_1\kappa_2(1+\gamma)}{\epsilon}}}\rd(t)
%    =\bigO\prns{\sqrt{\frac{\max(d_1,d_2)}{n}}\delta\log(1/\delta)}. 
%\end{align*}
%Thus, from Lemma \ref{lem:critical_basic}, the critical inequality is satisfied with $\eta_n=\tilde O(\sqrt{\max(d_1,d_2)/n})$. 
%\end{proof}

\begin{proof}[Proof of Lemma \ref{lem:vc_classes}]


We calculate 
\begin{align*}
      \frac{1}{\sqrt{n}}\int^{\eta}_{0}\sqrt{\log  \Ncal(t;\Gcal_q),\|\cdot\|_n)}\rd t.
\end{align*}
This is upper-bounded by 
\begin{align*}
     O\prns{ \frac{\log(n)}{\sqrt{n}}\int^{\eta}_{0}\sqrt{\max(V(\Wbbb),V(\Qbbb))\log(1/t) }\rd t }. 
\end{align*}
To prove this, we calculate 
\begin{align*}
      \frac{1}{\sqrt{n}}\int^{\eta}_{0}\sqrt{\log  \Ncal(t;\Gcal(\Wbbb,\Qbbb)),\|\cdot\|_n)}\rd t.
\end{align*}

Recall the empirical $L^2$-norm as $\|f(\cdot)\|_n= \{1/n\sum_if(s^i,a^i)^2\}^{1/2}$, $L^{\infty}$-norm as $\|\cdot\|_{n,\infty}=\max_{i}|f(s^i,a^i)|$. In addition, we define $\|f(\cdot)\|'_{n,\infty}\coloneqq \max_i| f(s'^i)|$, $\|f(\cdot)\|'_{n}\coloneqq \{ 1/n\sum_i f(s'^i)^2\}^{1/2}$. Then, from Lemma \ref{lem:dudley} (Dudley integral),
\begin{align*}
    & \ts\lesssim \int^{\eta}_0\sqrt{\frac{\log \Ncal(t,\Gcal(\Wbbb,\Qbbb),\|\cdot\|_n)}{n}}\rd\mu(t)\\
    &\ts \leq \int^{\eta}_0\sqrt{\frac{\log \Ncal(t,\Gcal(\Wbbb,\Qbbb),\|\cdot\|_{n,\infty})}{n}}\rd\mu(t)\\
     &\ts \leq\int^{\eta}_0\sqrt{\frac{\log \Ncal(t/\{(3(1+\gamma)C_{\Qbbb}\},\Wbbb,\|\cdot\|_{n,\infty})}{n}}+\sqrt{\frac{\log \Ncal(t/\{3C_{\Wbbb}\},\Qbbb,\|\cdot\|_{n,\infty})}{n}}+\sqrt{\frac{\log \Ncal(t/\{3\gamma C_{\Wbbb}\},\Vbbb,\|\cdot\|'_{n,\infty})}{n}} \rd\mu(t) \\ 
          &\ts \leq \int^{\eta}_0\sqrt{\frac{\log \Ncal(t/\{3(1+\gamma)C_{\Qbbb}\},\Wbbb,\sqrt{n}\|\cdot\|_{n})}{n}}+\sqrt{\frac{\log \Ncal(t/\{(3 C_{\Wbbb}\},\Qbbb,\sqrt{n}\|\cdot\|_{n})}{n}}+\sqrt{\frac{\log \Ncal(t/\{3\gamma C_{\Wbbb}\},\Vbbb,\sqrt{n}\|\cdot\|'_{n})}{n}} \rd\mu(t).
\end{align*}
From the second line to the third line, we use the same argument as the proof of Lemma \ref{lem:covering_G}: 
\begin{align*}
    &\ts \log \Ncal(t,\Gcal(\Wbbb,\Qbbb),\|\cdot\|_{n,\infty})\\
    &\ts \leq \log \Ncal(t/\{3(1+\gamma)C_{\Qbbb}\},\Wbbb,\|\cdot\|_{n,\infty})+ \log \Ncal(t/\{3 C_{\Wbbb}\},\Qbbb,\|\cdot\|_{n,\infty})\\
    &+\log \Ncal(t/\{3\gamma C_{\Wbbb}\},\Vbbb,\|\cdot\|'_{n,\infty}), 
\end{align*}
and $\sqrt{a+b+c}\leq \sqrt{a}+\sqrt{b}+\sqrt{c}$. From the third line to the fourth line, we use $\|\cdot\|_{n,\infty}\leq \sqrt{n}\|\cdot\|_{n} $. 
Then, 
\begin{align*}
    \ts  &\frac{1}{\sqrt{n}}\int^{\eta}_{0}\sqrt{\log  \Ncal(t;\Gcal(\Wbbb,\Qbbb)),\|\cdot\|_n)}\rd t\\
 &\ts O\prns{ \frac{\log(n)}{\sqrt{n}}\int^{\eta}_{0}\sqrt{\max(V(\Wbbb),V(\Qbbb))\log(1/t) }\rd t } \\ 
     &=O\prns{ \sqrt{\max(V(\Wbbb),V(\Qbbb))}\frac{\log(n)}{\sqrt{n}}\eta \log(1/\eta)}.  
\end{align*}
Thus, 
\begin{align*}
    \ts  \frac{1}{\sqrt{n}}\int^{\eta}_{0}\sqrt{\log  \Ncal(t;\Gcal_q),\|\cdot\|_n)}\rd t.
\end{align*}
is similarly upper-bounded. 


Finally, from Lemma \ref{lem:critical_basic}, the critical inequality becomes 
\begin{align*}
    \sqrt{\max(V(\Wbbb),V(\Qbbb))}\frac{\log(n)}{\sqrt{n}}\eta \log(1/\eta)\leq \eta^2. 
\end{align*}
This inequality is satisfied with $\eta=\tilde O(\sqrt{\max(V(\Wbbb),V(\Qbbb))/n})$. 
\end{proof}




\begin{proof}[Proof of Lemma \ref{lem:nonpara_critical}]
We use Lemma \ref{lem:critical_basic}. We consider the critical radius of $\Fcal$ s.t. 
\begin{align*}
    \log \Ncal(\tau;\Fcal,\|\cdot\|_{\infty})=(1/\tau)^{p}. 
\end{align*}
When $p\leq 2$, the critical inequality becomes
\begin{align*}
    \frac{2}{2-p}n^{-1/2}\eta^{1-0.5p}\leq \eta^2. 
\end{align*}
When $\eta=\Theta(n^{-1/(2+p)})$, this is satisfied. 

When $p=2$,  the critical inequality becomes
\begin{align*}
   \frac{1}{\sqrt{n}}\{\log (\eta)-\log(\eta^2/2\|\Fcal\|_{\infty})\}\leq \eta^2. 
\end{align*}
This is satisfied when $\eta=\Theta(n^{-1/4}\log n )$.

When $p\geq 2$,  the critical inequality becomes
\begin{align*}
        \frac{2}{p-2}n^{-1/2}\eta^{-p+2}\leq \eta^2. 
\end{align*}
This is satisfied when $\eta=\Theta(n^{-1/(2p)})$.

We apply the above analysis to our situation using the fact that the covering number of $G_q$ is upper-bounded as in the Lemma \ref{lem:covering_G}. 
Then, the proof is immediately concluded. 
\end{proof}

\begin{proof}[Proof of \cref{thm:sieve_rate}]
We consider $q_0 \in \Qbbb$ which will be specified later. From \cref{thm:agnostic_fast_q}, we obtain
\begin{align}
    \|\Tcal_\gamma ( \hat{q} - q_{\pi^e})\|_2 = O\prns{\eta + \epsilon_n + \frac{\|\Tcal_\gamma(q_{\pi^e} - q_0)\|_2^2}{\eta} + \|\Tcal_\gamma(q_{\pi^e} - q_0)\|_2}, \label{ineq:basic_sieve}
\end{align}
where $\eta$ is the maximum of critical radiuses of $\Wbbb$ and $\Gcal_q$, and $\epsilon_n = \sup_{q \in \Qbbb} \inf_{w \in \Wbbb} \|w - \Tcal_\gamma (q-q_0)\|_2$. We will bound each term in the right hand side of \eqref{ineq:basic_sieve}.

First. from Lemma \ref{lem:vc_classes}, $\eta=\tilde O(\sqrt{k_n/n})$. Next, we take $q_0$ s.t.
\begin{align*}
     \|\Tcal_\gamma(q_{\pi^e} - q_0)\|_2\leq (1+\gamma)\|q_{\pi^e} - q_0\|_{\infty})=O(k^{-p/d}_n). 
\end{align*}
from the assumption. 

Next, we show $\epsilon_n=O(k^{-p/d}_n)$. To do that, we check 
\begin{align*}
    \gamma \E_{s'\sim P_{S'|S,A}(s'|\cdot)}[-q(s',\epol)+q_0(s',\epol)]\in \Wcal^{p}_{2\gamma C_{\Qbbb}K}(I^d). 
\end{align*}
Let $\|\cdot\|_b$ be a \Holder\,norm. By the assumption on the density $P_{S'|S,A}(s'|\cdot)$, we can bound the \Holder\,norm of $ \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e)]$
\begin{align*}
    \|\E_{s'\sim P_{S'|S,A}(s'|\cdot)}[q(s',\epol)]\|_{b}&=\left\|\int_{[0,1]^d}q(s',\epol)P_{S'|S,A}(s'|\cdot)\rd s'\right\|_b \\
    &\leq C_{\Qbbb}\left\|\int_{[0,1]^d} P_{S'|S,A}(s'|\cdot)\rd s'\right\|_b\leq C_{\Qbbb}\int_{[0,1]^d} \|P_{S'|S,A}(s'|\cdot)\|_b\rd s'\\
    &\leq C_{\Qbbb}\int_{[0,1]^d} K\rd s'=C_{\Qbbb}K. 
\end{align*}
Then, for any $q\in \Qbbb$, we can take $w'\in W'$ s.t. 
\begin{align*}
    \|w''- \gamma \E_{s'\sim P_{S'|S,A}}[-q(s',\epol)+q_0(s',\epol)]\|_{\infty}= O(k^{-p/d}_n). 
\end{align*}
Thus, by defining $w'=w''-(q-q_0)$, we can take $w'\in \Wbbb$ s.t. 
\begin{align*}
    \|w'-\Tcal_{\gamma}(q-q_0)\|_2\leq     \|w'-\Tcal_{\gamma}(q-q_0)\|_{\infty}=O(k^{-p/d}_n). 
\end{align*}

Finally, the error is 
\begin{align*}
         \|\Tcal_\gamma ( \hat{q} - q_{\pi^e})\|_2&= O\prns{\sqrt{k_n/n}+k^{-p/d}_n+\frac{k^{-2p/d}_n}{\sqrt{k_n/n}}  }\\
         &=\tilde O(n^{-p/(2p+d)}). \tag{Taking balance of both terms}
\end{align*}

\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:neural_policy_rate}]

We consider $q_0 \in \Qbbb$ which will be specified later. From \ref{thm:agnostic_fast_q}, we obtain
\begin{align}
    \|\Tcal_\gamma ( \hat{q} - q_{\pi^e})\|_2 = O\prns{\eta + \epsilon_n + \frac{\|\Tcal_\gamma(q_{\pi^e} - q_0)\|_2^2}{\eta} + \|\Tcal_\gamma(q_{\pi^e} - q_0)\|_2}, \label{ineq:basic_nn}
\end{align}
where $\eta$ is the maximum of critical radiuses of $\Wbbb$ and $\Gcal_q$, and $\epsilon_n = \sup_{q \in \Qbbb} \inf_{w \in \Wbbb} \|w - \Tcal_\gamma (q-q_0)\|_2$. We will bound each term in the right hand side of \eqref{ineq:basic_nn}.


For the third and fourth terms, we consider an approximation power by fixing $q_0$. We set $q_0 = \argmin_{q \in \Qbbb} \|q - q_{\pi^e}\|_\infty$. By Lemma \ref{lem:yaro} and boundedness of $\Tcal_\gamma$, we obtain
\begin{align*}
    \|\Tcal_\gamma(q_{\pi^e} - q_0)\|_2  \leq (1+\gamma )\|q_{\pi^e} - q_0\|_\infty = \tilde{O}(\Omega^{-p/d}).
\end{align*}
By this result, we bound the third and fourth terms in \eqref{ineq:basic_nn} by
\begin{align*}
    \tilde{O}(\eta^{-1}\Omega^{-2p/d} + \Omega^{-p/d}).
\end{align*}

About the second term $\epsilon_n$ in \eqref{ineq:basic_nn}, we fix $q \in \Qbbb$ arbitrary and consider an explicit form of $\Tcal_\gamma (q-q_0)$ as
\begin{align*}
    \Tcal_\gamma (q-q_0) = \gamma \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e) - q_0(s', \pi^e)] -(q-q_0).
\end{align*}
We define $\Wbbb'$ as a set of neural network with $L$ layers and $W$ parameters.
By the assumption, $\Wbbb' \supseteq \Qbbb$ holds, hence $q,q_0 \in \Wbbb'$ is satisfied.
Let $\|\cdot\|_b$ be a Sobolev norm. By the assumption on the density $P_{S'|S,A}(s'|\cdot)$, we can bound the Sobolev norm of $ \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e)]$ as
%we can state that $\gamma \mathbb{E}_{s' \sim P(s'|\cdot)}[q(s', \pi^e) - q_0(s', \pi^e)] \in \Wcal_K^p(I_d)$. \masa{check}
%{\blockedit 
%$\mu$ is Lebesgue measure on $[0,1]^d$. 
\begin{align*}
    \|E_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s',\epol)]\|_{b}&=\left\|\int_{[0,1]^d}q(s',\epol)P_{S'|S,A}(s'|\cdot)\rd s'\right\|_b \\
    &\leq C_{\Qbbb}\left\|\int_{[0,1]^d} P_{S'|S,A}(s'|\cdot)\rd s'\right\|_b\leq C_{\Qbbb}\int_{[0,1]^d} \|P_{S'|S,A}(s'|\cdot)\|_b\rd s'\\
    &\leq C_{\Qbbb}\int_{[0,1]^d} K\rd s'=C_{\Qbbb}K. 
\end{align*}
Thus, 
$\gamma \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e) - q_0(s', \pi^e)] \in \Wcal_{2\gamma C_{\Qbbb}K}^p(I_d)$
%}
Hence, we pick $w' \in \Wbbb'$ as
\begin{align*}
    \|w' -  \gamma \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e) - q_0(s', \pi^e)]\|_\infty = \tilde{O}(\Omega^{-p/d}),
\end{align*}
by Lemma \ref{lem:yaro}.
We set $w \in \Wbbb$ as $w=w' - q - q_0$ and obtain
\begin{align*}
    \|w - \Tcal_\gamma(q-q_0)\|_2 &= \|w' - \gamma \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e) - q_0(s', \pi^e)]\|_2 \\
    &\leq \|w' -  \gamma \mathbb{E}_{s' \sim P_{S'|S,A}(s'|\cdot)}[q(s', \pi^e) - q_0(s', \pi^e)]\|_\infty = \tilde{O}(\Omega^{-p/d}).
\end{align*}
Hence, we have
\begin{align*}
    \epsilon_n = \tilde{O}(\Omega^{-p/d}).
\end{align*}
Combining the results with \eqref{ineq:basic_nn}, we obtain
\begin{align}
    \|\Tcal_\gamma ( \hat{q} - q_{\pi^e})\|_2 \lesssim (1+C_1)^2 \eta +\tilde{O}(\eta^{-1}\Omega^{-2p/d} + \Omega^{-p/d}). \label{ineq:basic_nn2}
\end{align}

Next, We derive an explicit order of $\eta$ by deriving a critical radius of $\Wbbb$.
By Lemma \ref{lem:covering_neural}, we have
\begin{align*}
    \log \Ncal(\varepsilon, \Wbbb, \|\cdot\|_\infty) \leq \Omega\log \left( \frac{ 2(L+1)B^{(L+1)} (3W+1)^{(L+1)}}{\varepsilon} \right) \lesssim  \Omega L \log\left( \frac{LB\Omega}{ \varepsilon} \right).
\end{align*}
To the end, we derive the following local Rademacher complexity of the star-hull of $\Wbbb$ as Lemma \ref{lem:support2},
\begin{align*}
    &\frac{1}{\sqrt{n}}\int_{0}^\delta \sqrt{\log \Ncal( t, \mathrm{star}(\Wbbb), \|\cdot\|_n)} dt \\
    &\lesssim \frac{1}{\sqrt{n}}\int_{0}^\delta \sqrt{\log \Ncal( t, \mathrm{star}(\Wbbb), \|\cdot\|_\infty)} dt \\
    & \leq \frac{1}{\sqrt{n}}\int_{0}^\delta \sqrt{ \log (1/t) + \log \Ncal( t/2, \Wbbb, \|\cdot\|_\infty)} dt\\
    &\lesssim \frac{1}{\sqrt{n}}\int_{0}^\delta \sqrt{\log (1/t)} dt +  \sqrt{\frac{\Omega L}{n}} \int_{0}^\delta \sqrt{\log (LB\Omega/t)} dt\\
    &=\bigO\prns{ \sqrt{\frac{\Omega L}{n}}\delta\log(LB\Omega/\delta))},
\end{align*}
for any $\delta > 0$.
The second inequality follows Lemma 4.5 in \cite{mendelson2002improving} for a covering number of a star-hull of sets.
We note that the lemma in \cite{mendelson2002improving} holds regardless of the choice of norms.
By setting
\begin{align*}
    \eta = \tilde O\prns{\sqrt{\frac{\Omega L}{n}}},
\end{align*}
the  critical inequality of $\Wbbb$ is satisfied. Similarly, the  critical inequality of $\Gcal_q$ is satisfied for this $\eta$ utilizing Lemma \ref{lem:covering_G}. 

We substitute $\eta$ into \eqref{ineq:basic_nn2} and achieve
\begin{align*}
    \|\Tcal_\gamma ( \hat{q} - q_{\pi^e})\|_2 \lesssim \tilde O\prns{\sqrt{\frac{\Omega L}{n}}} +\tilde{O}(n^{1/2} L^{1/2} \Omega^{-2p/d - 1/2} + \Omega^{-p/d})
\end{align*}
Then, by setting $L = \Theta(\log n)$ and $W=\Theta(n^{d/(2p + d)})$, the statement is concluded. 
\end{proof}




%For a matrix $A$, let $\|A\|_\sigma$ is a spectral norm and $\|A\|_{2,1} = {\sum_i \sqrt{\sum_j A_{i,j}^2}}$ is a $2,1$-norm.

%\begin{lemma}[Theorem 3.3 in \cite{bartlett2017spectrally}]
%    Let $\mathcal{F}_{NN}$ be a set of functions by a neural network with $L$ layers and activation function which is $1$-Lipschitz continuous.
%    Further, let $A_\ell$ be a weight matrix of an $\ell$-th layers for $\ell = 1,...,L$ and assume that $\|A_\ell\|_{\sigma} \leq M_\sigma(\ell)$ and $\|A_\ell^\top\|_{2,1} \leq M_{2,1}(\ell)$ with bounds $M_\sigma(\ell)$ and $M_{2,1}(\ell)$.
%    Then, for $\varepsilon > 0$, we have
%    \begin{align*}
%        \log \mathcal{N}(\varepsilon, \mathcal{F}_{NN}, \|\cdot\|_2) \leq  \frac{ n \max_x\|x\|_2  \prod_{\ell=1}^L M_\sigma(\ell)^2 (\sum_{\ell = 1^L} (M_{2,1}(\ell)/M_{\sigma}(\ell) )^{2/3} )^3}{\varepsilon^2}.
%    \end{align*}
%\end{lemma}

%\imaizumi{We may obtain two types of bounds}:
%\begin{align*}
%    O\left( \frac{B \sqrt{\log L} \prod_{\ell=1}^L M(\ell)}{\sqrt{n}} \right) \mbox{~or~} O\left( \frac{B  (\prod_{\ell=1}^L M(\ell))^2}{n} \right)
%\end{align*}
%$B := \max_x \|x\|_2$: input scale, $M(\ell) \geq \|A_\ell\|$: norm bound of a parameter matrix $A_\ell$ in $\ell$-th layer


==> proof/proof_mdl.tex <==
\begin{proof}[Proof of \cref{thm:generalization2}]
We only consider the case of $\hat J^{\MDL}_{w1}$. The statements regarding the other estimators are similarly proved. 

In this proof, let 
\begin{align*}
    f(s,a,r,s';w,q) \coloneqq w(s,a)\{r-q(s,a)+\gamma q(s',\epol)\}+\E_{d_0}[q(s_0,\epol)]. 
\end{align*}
and $\hat J^{\MDL}_{w1}=\E_n[f(\hat w,\hat q)]$. First, we bound the difference of $\E[f(\hat w,\hat q)]$ and $J(\epol)$. 

From Lemma \ref{lem:minimax}, we have 
\begin{align*}
&\ts \E[w(s,a)\{r-q(s,a)+\gamma v(s')\}]+(1-\gamma)\E_{s_0}[v(s_0)]\\
&\ts =\E[\{w(s,a)-w_{\epol}(s,a)\}\{-q(s,a)+q_{\epol}(s,a)+\gamma v(s')-\gamma v_{\epol}(s)\}]+J(\epol)\\
&\ts=\E[\{w(s,a)-w_{\epol}(s,a)\}\{\Tcal_{\gamma} q(s,a)- \Tcal_{\gamma} q_{\epol}(s,a)\}]+J=\langle w-w_{\epol},\Tcal_{\gamma} q- \Tcal_{\gamma} q_{\epol}\rangle +J(\epol)\\
&\ts =\langle \Tcal'_{\gamma}(w-w_{\epol}),(q- q_{\epol})\rangle +J(\epol) =\E[\{\Tcal_{\gamma}' w(s,a)-\Tcal_{\gamma}' w_{\epol}(s,a)\}\{q(s,a)- q_{\epol}(s,a)\}]+J(\epol). 
\end{align*}

We prove a statement in the three steps. 
\\ 
\textbf{Step 1 }

Take $w^{\dagger}$ s.t. 
\begin{align*}
    J(\epol)=\E[f(s,a,r,s';w^{\dagger},q)]. 
\end{align*}
for any $q\in \Qbbb$. The function $w_{\epol}$ satisfies this $w^{\dagger}$.  Then, 
\begin{align*}
& \E[f(\hat w,\hat q)]-J= \E[f(\hat w,\hat q)]-\E[f(w^{\dagger},\hat q)]\\
&= \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+ \E_n[f(\hat w,\hat q)]-\E_n[f(w^{\dagger},\hat q)]+\E_n[f(w^{\dagger},\hat q)]-\E[f(w^{\dagger},\hat q)]\\
&\leq \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+\E_n[f(w^{\dagger},\hat q)]-\E[f(w^{\dagger},\hat q)]\\
&\leq 2|\sup_{w\in \Wbbb}\sup_{q\in \Qbbb}(\E[f(w, q)]-\E_n[f(w, q)])|. 
\end{align*}
We use $ \E_n[f(\hat w,\hat q)]\leq \E_n[f(w^{\dagger},\hat q)]$. 

\textbf{Step 2 }

Take $q^{\dagger}\in \Qbbb$ s.t. 
\begin{align*}
    J(\epol)=\E[f(s,a,r,s';w,q^{\dagger})] 
\end{align*}
for any $w\in \Wbbb$. The function $q_{\epol}$ satisfies this $q^{\dagger}$.  Then, 
\begin{align*}
& \E[f(\hat w,\hat q)]-J= \E[f(\hat w,\hat q)]-\E[f(\hat w,q^{\dagger})]\\
&= \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+ \E_n[f(\hat w,\hat q)]-\E_n[f(\hat w, q^{\dagger})]+\E_n[f(\hat w,q^{\dagger})]-\E[f(\hat w,q^{\dagger})]\\
&\geq \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+\E_n[f(\hat w,q^{\dagger})]-\E[f(\hat w,q^{\dagger})]\\
&= -2|\sup_{w\in \Wbbb}\sup_{q\in \Qbbb}(\E[f(w,q)]-\E_n[f(w,q)])|. 
\end{align*}
We use $\ts \E_n[f(\hat w,\hat q)]\geq \E_n[f(\hat w, q^{\dagger})]$. 

\textbf{Step 3 }

Combining results in Step 1 and Step 2, we have 
\begin{align*}\ts
    |\E[f(\hat w,\hat q)]-J|&\leq  \ts |\sup_{w\in \Wbbb,q\in \Qbbb}(\E_n-\E)[w(s,a)\{r-q(s,a)+\gamma v(s')\}]|. 
\end{align*}
In addition, 
\begin{align*}\ts
    |\E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]|&\leq |\sup_{w\in \Wbbb,q\in \Qbbb}(\E_n-\E)[w(s,a)\{r-q(s,a)+\gamma v(s')\}]. 
\end{align*}
Thus, with probability $1-\delta$, the difference $|\E_n[f(\hat w,\hat q)]-J(\epol)|$ is upper-bounded by
\begin{align*}
  R_{\max}\Rcal_n(\Wbbb)+\Rcal_n(\Gcal(\Wbbb,\Qbbb))+C_{\Wbbb}(R_{\max}+C_{\Qbbb})\sqrt{\frac{\log(2/\delta)}{n}}. 
\end{align*}
up to universal constants. 
\end{proof}





\begin{proof}[Proof of \cref{thm:recovery2}  ]

First, we prove the statement regarding weight functions. Then, we prove the statement regarding q-functions. 

\textbf{W-functions}

We consider the following estimator:
\begin{align*}
   &\hat w= \argmin_{w\in \Wbbb}\max_{q\in \Qbbb}\E_n[   f(s,a,r,s';w,q) ],\\
 & f(s,a,r,s';w,q) \coloneqq w(s,a)\{r-q(s,a)+\gamma q(s',\epol)\}+\E_{s_0}[q(s_0,\epol)]. 
\end{align*}
We write the solution to $(\hat w,\hat q)$. From the assumption $C_{\xi}\Tcal'_{\gamma}(\Wbbb-w_{\epol})\subset (\Qbbb-q_{\epol})$, we have 
\begin{align*}
    &\E[\{\Bcal\hat w-\hat w\}^2]=\E[\{\Tcal'_{\gamma}(\hat w-w_{\epol})\}^2]\leq C^{-1}_{\xi}\max_{q\in \Qbbb}\E[\Tcal'_{\gamma}(\hat w-w_{\epol})(q-q_{\epol})]=C^{-1}_{\xi}\E[\Tcal'_{\gamma}(\hat w-w_{\epol})(\tilde q-q)],\\
    &\tilde q=\argmax_{q\in \Qbbb}\E[\Tcal'_{\gamma}(\hat w-w_{\epol})(q-q_{\epol}) ]. 
\end{align*}
Thus, if we can bound $\E[\Tcal'_{\gamma}(\hat w-w_{\epol})(\tilde q-q)]$, the convergence rate is obtained. 


As a first step, we bound  $\E[\Tcal'_{\gamma}(\hat w-w_{\epol})(\hat q-q)]$. This is actually showed in the proof of \cref{thm:generalization2}:
\begin{align*}
\E[\Tcal'_{\gamma}(\hat w-w_{\epol})(\hat q-q_{\epol})] \leq |\E[f(\hat w,\hat q)]-J|
     \leq 2\sup_{w\in \Wbbb,q\in \Qbbb}|(\E_n-\E)[f(w,q)]|. 
\end{align*}
noting the assumption in \cref{thm:generalization2} is satisfied. 
Second, we have 
\begin{align*}
    &\E[\Tcal'_{\gamma}(\hat w-w_{\epol}))(\tilde q-q)]-\E[\Tcal'_{\gamma}(\hat w-w_{\epol}))(\hat q-q_{\epol})]\\
&=\E[f(\hat w,\tilde q)]-    \E[f(\hat w,\hat q)] \\
&=\E[f(\hat w,\tilde q)]-\E_n[f(\hat w,\tilde q)] +\E_n[f(\hat w,\tilde q)] -\E_n[f(\hat w,\hat q)]+\E_n[f(\hat w,\hat q)]   \E[f(\hat w,\hat q)] \\
&\leq \E[f(\hat w,\tilde q)]-\E_n[f(\hat w,\tilde q)] +\E_n[f(\hat w,\hat q)] - \E[f(\hat w,\hat q)]\\
& \leq 2\sup_{w\in \Wbbb,q\in \Qbbb}|(\E_n-\E)[f(w,q)]|. 
\end{align*}
Here, we use $\E_n[f(\hat w,\tilde q)] \leq \E_n[f(\hat w,\hat q)]$. Then, 
\begin{align*}
  \E[(\Bcal'\hat w-\hat w)^2] \leq 4C^{-1}_{\xi}\sup_{w\in \Wbbb,q\in \Qbbb}|(\E_n-\E)[f(w,q)]|. 
\end{align*}




\textbf{Q-functions }
We consider the following estimator:
\begin{align*}
   &\hat q= \argmin_{q\in \Qbbb}\max_{w\in \Wbbb}\E_n[   f(s,a,r,s';w,q) ],\\
 & f(s,a,r,s';w,q) \coloneqq w(s,a)\{r-q(s,a)+\gamma q(s',\epol)\}+\E_{d_0}[q(s_0,\epol)]. 
\end{align*}
We write the solution to $(\hat q,\hat w)$.
%Importantly, we have 
%\begin{align*}
%    \E[ f(s,a,r,s';w,q)]=\E[(w-w_{\epol})\Tcal_{\gamma}(q-q_{\epol})]+J. 
%\end{align*}
From the assumption $C_{\xi}\Tcal_{\gamma}(\Qbbb-q_{\epol})\subset (\Wbbb-w_{\epol})$, we have 
\begin{align*}
    &\E[\{\Bcal\hat q-\hat q\}^2]=\E[\{\Tcal_{\gamma}(\hat q-q_{\epol})\}^2]\leq C^{-1}_{\xi}\max_{w\in \Wbbb}\E[(w-w_{\epol})\Tcal_{\gamma}(\hat q-q_{\epol})]=C^{-1}_{\xi}\E[(\tilde w-w)\Tcal_{\gamma}(\hat q-q_{\epol})],\\
    &\tilde w=\argmax_{w\in \Wbbb}\E[(w-w_{\epol})\Tcal_{\gamma}(\hat q-q_{\epol}) ]. 
\end{align*}
Thus, if we can bound $ \E[(\tilde w-w)\Tcal_{\gamma}(\hat q-q_{\epol})]$, the convergence rate is obtained. 


As a first step, we bound  $ \E[(\hat w-w_{\epol})\Tcal_{\gamma}(\hat q-q_{\epol})]$. This is actually showed in the proof of \cref{thm:generalization}:
\begin{align*}
     \E[(\hat w-w_{\epol})\Tcal_{\gamma}(\hat q-q_{\epol})]\leq |\E[f(\hat w,\hat q)]-J|
     \leq 2\sup_{w\in \Wbbb,q\in \Qbbb}|(\E_n-\E)[f(w,q)]|
\end{align*}
noting the assumption in \cref{thm:generalization} is satisfied. 
Second, we have 
\begin{align*}
     & \E[(\tilde w-w)\Tcal_{\gamma}(\hat q-q_{\epol})]-  \E[(\hat w-w_{\epol})(\Tcal_{\gamma}\hat q-q_{\epol})]\\
 &= \E[f(\tilde w,\hat q)  ]- \E[f(\hat w,\hat q)  ]\\
 &=  \E[f(\tilde w,\hat q)  ]-\E_n[f(\tilde w,\hat q)  ]+\E_n[f(\tilde w,\hat q)  ] -\E_n[f(\hat w,\hat q)  ]+\E_n[f(\hat w,\hat q)  ]-\E[f(\hat w,\hat q)  ]\\
 &\leq \E[f(\tilde w,\hat q)  ]-\E_n[f(\tilde w,\hat q)  ]+\E_n[f(\hat w,\hat q)  ]-\E[f(\hat w,\hat q)]\\
& \leq 2\sup_{w\in \Wbbb,q\in \Qbbb}|(\E_n-\E)[f(w,q)]|. 
\end{align*}
Here, we use $\E_n[f(\tilde w,\hat q)  ] \leq \E_n[f(\hat w,\hat q) ]$. 
Therefore,
\begin{align*}
  \E[(\Bcal\hat q-\hat q)^2] \leq 4C^{-1}_{\xi}\sup_{w\in \Wbbb,q\in \Qbbb}|(\E_n-\E)[f(w,q)]|. 
\end{align*}


\end{proof}



==> proof/proof_not_used.tex <==
\begin{proof}[Proof of \cref{thm:allow_mis2}]
We only consider the case of $\hat J^{\MDL}_{w1}$. The statements regarding the other estimators are similarly proved. In this proof, let 
\begin{align*}
    f(s,a,r,s';w,q) \coloneqq w(s,a)\{r-q(s,a)+\gamma q(s',\epol)\}+\E_{d_0}[q(s_0,\epol)]. 
\end{align*}
and $\hat J^{\MDL}_{w1}=\E_n[f(\hat w,\hat q)]$. First, we bound the difference of $\E[f(\hat w,\hat q)]$ and $J(\epol)$. 

From Lemma \ref{lem:minimax}, we have 
\begin{align*}
&\ts \E[w(s,a)\{r-q(s,a)+\gamma v(s')\}]+(1-\gamma)\E_{s_0}[v(s_0)]\\
&\ts =\E[\{w(s,a)-w_{\epol}(s,a)\}\{-q(s,a)+q_{\epol}(s,a)+\gamma v(s')-\gamma v_{\epol}(s)\}]+J(\epol)\\
&\ts=\E[\{w(s,a)-w_{\epol}(s,a)\}\{\Tcal_{\gamma} q(s,a)- \Tcal_{\gamma} q_{\epol}(s,a)\}]+J=\langle w-w_{\epol},\Tcal_{\gamma} q- \Tcal_{\gamma} q_{\epol}\rangle +J(\epol)\\
&\ts =\langle \Tcal'_{\gamma}(w-w_{\epol}),(q- q_{\epol})\rangle +J(\epol) =\E[\{\Tcal_{\gamma}' w(s,a)-\Tcal_{\gamma}' w_{\epol}(s,a)\}\{q(s,a)- q_{\epol}(s,a)\}]+J(\epol). 
\end{align*}

We prove a statement in the three steps. 

\textbf{Step 1 }\\

Take $w^{\dagger}$ s.t. 
\begin{align*}
w^{\dagger}=\argmin_{w\in \Wbbb}\max_{q\in \Qbbb}\E[f(s,a,r,s';w,q)]. 
\end{align*}
Then, 
\begin{align*}
& \E[f(\hat w,\hat q)]-\E[f(w^{\dagger},\hat q)]\\
&= \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+ \E_n[f(\hat w,\hat q)]-\E_n[f(w^{\dagger},\hat q)]+\E_n[f(w^{\dagger},\hat q)]-\E[f(w^{\dagger},\hat q)]\\
&\leq \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+\E_n[f(w^{\dagger},\hat q)]-\E[f(w^{\dagger},\hat q)]\\
&\leq 2|\sup_{w\in \Wbbb}\sup_{q\in \Qbbb}(\E[f(w, q)]-\E_n[f(w, q)])|. 
\end{align*}
from $\E_n[f(\hat w,\hat q)]\leq \E_n[f(w^{\dagger},\hat q)]$. 
Thus, 
\begin{align*}
\E[f(\hat w,\hat q)]-J&=\E[f(\hat w,\hat q)]-\{\E[f(w^{\dagger},\hat q)]-\E[\{w^{\dagger}-w_{\epol}\}\Tcal_{\gamma}(\hat q-q_{\epol}) ] \}\\
&\leq \E[f(\hat w,\hat q)]-\E[f(w^{\dagger},\hat q)]+\min_{w\in \Wbbb}\max_{q\in \Qbbb}\E[\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})]\\
&\leq 2|\sup_{w\in \Wbbb}\sup_{q\in \Qbbb}(\E[f(w, q)]-\E_n[f(w, q)])|+\min_{w\in \Wbbb}\max_{q\in \Qbbb}\E[\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})] \tag{Proof of \cref{thm:generalization2}}. 
\end{align*}

\textbf{Step 2 }

Take $q^{\dagger}$ s.t. 
\begin{align*}
   q^{\dagger}=\argmin_{q\in \Qbbb}\max_{w\in \Wbbb}\E[-f(s,a,r,s';w,q)] 
\end{align*}
Then, 
\begin{align*}
& \E[f(\hat w,\hat q)]-\E[f(\hat w,q^{\dagger})]\\
&= \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+ \E_n[f(\hat w,\hat q)]-\E_n[f(\hat w, q^{\dagger})]+\E_n[f(\hat w,q^{\dagger})]-\E[f(\hat w,q^{\dagger})]\\
&\geq \E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]+\E_n[f(\hat w,q^{\dagger})]-\E[f(\hat w,q^{\dagger})]\\
&= -2|\sup_{w\in \Wbbb}\sup_{q\in \Qbbb}(\E[f(w,q)]-\E_n[f(w,q)])|. 
\end{align*}
We use $  \E_n[f(\hat w,\hat q)]\geq \E_n[f(\hat w, q^{\dagger})]$. 
Thus, 
\begin{align*}
    \E[f(\hat w,\hat q)]-J&=    \E[f(\hat w,\hat q)]-\{\E[f(\hat w, q^{\dagger})]-\E[\{\hat w-w_{\epol}\}\Tcal_{\gamma}(q^{\dagger}-q_{\epol}) ]\}\\
    &= \E[f(\hat w,\hat q)]-\E[f(\hat w,q^{\dagger})]-\min_{q\in \Qbbb}\max_{w\in \Wbbb}\E[-\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})] \\
    &\geq -2|\sup_{w\in \Wbbb}\sup_{q\in \Qbbb}(\E[f(w,q)]-\E_n[f(w,q)])|-\min_{q\in \Qbbb}\max_{w\in \Wbbb}\E[-\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})]. 
\end{align*}

\textbf{Step 3 }

Combining results in Step 1 and Step 2, we have 
\begin{align*}
    |\E[f(\hat w,\hat q)]-J|&\leq  \ts 2|\sup_{w\in \Wbbb,q\in \Qbbb}(\E_n-\E)[w(s,a)\{r-q(s,a)+\gamma v(s')\}]|+\\
    &+\min_{q\in \Qbbb}\max_{w\in \Wbbb}\E[-\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})]+\min_{w\in \Wbbb}\max_{q\in \Qbbb}\E[\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})]. 
\end{align*}
In addition, 
\begin{align*}
    |\E[f(\hat w,\hat q)]-\E_n[f(\hat w,\hat q)]|&\leq |\sup_{w\in \Wbbb,q\in \Qbbb}(\E_n-\E)[w(s,a)\{r-q(s,a)+\gamma v(s')\}]. 
\end{align*}
Thus, with probability $1-\delta$, the difference $|\E_n[f(\hat w,\hat q)]-J(\epol)|$ is upper-bounded by
\begin{align*}
  &R_{\max}\Rcal_n(\Wbbb)+\Rcal_n(\Gcal(\Wbbb,\Qbbb))+C_{\Wbbb}(R_{\max}+C_{\Qbbb})\sqrt{\frac{\log(2/\delta)}{n}}+\\
  &+\min_{q\in \Qbbb}\max_{w\in \Wbbb}\E[-\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})]+\min_{w\in \Wbbb}\max_{q\in \Qbbb}\E[\{w-w_{\epol}\}\Tcal_{\gamma}(q-q_{\epol})]. 
\end{align*}
up to universal constants. 




\end{proof}
